Induce, Edit, Retrieve: Language Grounded Multimodal Schema for Instructional Video Retrieval

Schemata are structured representations of complex tasks that can aid artificial intelligence by allowing models to break down complex tasks into intermediate steps. We propose a novel system that induces schemata from web videos and generalizes them to capture unseen tasks with the goal of improving video retrieval performance. Our system proceeds in three major phases: (1) Given a task with related videos, we construct an initial schema for a task using a joint video-text model to match video segments with text representing steps from wikiHow; (2) We generalize schemata to unseen tasks by leveraging language models to edit the text within existing schemata. Through generalization, we can allow our schemata to cover a more extensive range of tasks with a small amount of learning data; (3) We conduct zero-shot instructional video retrieval with the unseen task names as the queries. Our schema-guided approach outperforms existing methods for video retrieval, and we demonstrate that the schemata induced by our system are better than those generated by other models.

==> tables/howtogen_results.tex <==
\begin{table*}[!t]
\centering
\resizebox{13cm}{!}{
\begin{tabular}{cc|cccccccc}
\Xhline{2\arrayrulewidth}
\multicolumn{2}{c|}{\textbf{Method}}    & \textbf{P@1}$\uparrow$ & \textbf{R@5}$\uparrow$ & \textbf{R@10}$\uparrow$ & \textbf{R@25}$\uparrow$ & \textbf{R@50}$\uparrow$ & \textbf{Mean r}$\downarrow$ & \textbf{Med r}$\downarrow$ & \textbf{MRR}$\uparrow$ \\ \hline
\multirow{2}{*}{}                                                          & MIL-NCE\cite{miech20endtoend} & 45.2 & 31.0 & 43.1 & 58.2 & 68.9 & 110.8  & 15.0  & .198     \\ \hline
\multirow{7}{*}{\STAB{\rotatebox[origin=c]{90}{Step Aggregation}}}         & T5*(FT)\cite{Lyu-et-al:2021} & 44.0 & 29.9 & 41.0 & 55.1 & 65.3 & 138.2 & 19.0 & .190     \\
                                                                          & GPT-2(FT) & 46.0 & 31.5 & 43.3 & 57.5 & 67.3 & 127.4 & 16.0 & .200    \\
                                                                          & GPT-3 & 49.3 & 33.3 & 45.7 & 60.5 & 70.9 & 103.7 & 13.0 & .211 \\
                                                                          & GOSC*\cite{Lyu-et-al:2021} & 54.7 & 37.0 & 49.8 & 64.9 & 74.4 & 92.0 & 11.0 & .231  \\
                                                                          & wikiHow & 51.9 & 35.4 & 47.8 & 62.8 & 72.1 & 103.4 & 11.0 & .222 \\
                                                                          & IER (Ours) & 54.4 & 37.3 & 50.1 & 64.8 & 74.4 & 90.1 & 10.0 & .231\\
                                                                          & IER$^3$ (Ours) & \textbf{55.0} & \textbf{37.4} & \textbf{50.6} & \textbf{65.7} & \textbf{75.2} & \textbf{88.6} & \textbf{10.0} & \textbf{.234}    \\ \cline{2-10}
                                                                          & Oracle & 56.5 & 38.0 & 50.8 & 65.2 & 74.9 & 95.9 & 10.0 & .237 \\ \Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{Retrieval Performance on Howto-GEN test set. (FT stands for fine-tuned, * represents the model has seen the ground truth schema of the tasks in the test set during training.)}
\label{howtogen_results}
\end{table*}

==> tables/matching_function_ablation.tex <==
\begin{table*}[!t]
\centering
\resizebox{15cm}{!}{%
\begin{tabular}{c|cccc|cccc|cccc}
\Xhline{2\arrayrulewidth}
\multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Generalization}\\ \textbf{Probability}\end{tabular}}} & \multicolumn{4}{c|}{\textbf{Howto-GEN}} & \multicolumn{4}{c|}{\textbf{COIN}} & \multicolumn{4}{c}{\textbf{Youccok2}} \\ \cline{2-13} 
                  & \textbf{P@1}$\uparrow$ & \textbf{R@5}$\uparrow$ & \textbf{R@10}$\uparrow$ & \textbf{Mean r}$\downarrow$ & \textbf{P@1}$\uparrow$ & \textbf{R@5}$\uparrow$ & \textbf{R@10}$\uparrow$ & \textbf{Mean r}$\downarrow$ & \textbf{P@1}$\uparrow$ & \textbf{R@5}$\uparrow$ & \textbf{R@10}$\uparrow$ & \textbf{Mean r}$\downarrow$ \\ \hline
$\max (\mathcal{G}_{txt}, \mathcal{G}_{vis})$   & 55.0    &  37.4   & 50.6    &  88.6     & 56.1    & 42.3    &  59.1    & 33.3   & 43.8  & 30.8   & 44.7    & 47.4      \\
$\mathcal{G}_{vis}$                             &  54.9   &  37.5   &  50.6    &  88.5     & 55.0    & 42.3    &  59.1    & 33.5   & 43.8  & 29.8   & 44.2    & 48.0   \\
$\mathcal{G}_{txt}$                             & 50.1    & 34.5    & 47.3     & 98.9       & 55.0    & 42.3    &  58.4    & 38.2   & 40.4      & 28.9   &  43.0   &  54.3      \\ \Xhline{2\arrayrulewidth}
\end{tabular}
}
\caption{Comparison over different ways to compute the generalization probability.}
\end{table*}

==> tables/wikihow_step_data.tex <==
\begin{table}[!t]
\centering
\resizebox{7.5cm}{!}{%
\begin{tabular}{ccc}
\hline
\textbf{Category}                  & \textbf{Tasks}                     & \textbf{Steps}                     \\ \hline
Computers and Electronics & 15.7k                     & 149.9k                    \\
Food and Entertaining     & 12.6k                     & 130.9k                    \\
Health                    & 12.4k                     & 168.4k                    \\
Home and Garden           & 10.4k                     & 122.6k                    \\
Hobbies and Crafts        & 9.8k                      & 98.1k                     \\
Arts and Entertainment    & 6.0k                      & 63.4k                     \\
Personal Care and Style   & 5.7k                      & 74.3k                     \\
Pets and Animals          & 4.1k                      & 54.6k                     \\
Sports and Fitness        & 3.0k                      & 34.2k                     \\
Cars \& Other Vehicles    & 2.6k                      & 26.0k                     \\ \hline
Total                     & \multicolumn{1}{l}{92.1k} & \multicolumn{1}{l}{1.04m} \\\hline
\end{tabular}
}
\caption{Number of tasks and steps within each category of wikiHow used for step labeling.}
\label{wiki-steps}
\end{table}
